Investigating Robustness of Dialog Models to Popular Figurative Language Constructs

Humans often employ figurative language use in communication, including during interactions with dialog systems. Thus, it is important for real-world dialog systems to be able to handle popular figurative language constructs like metaphor and simile. In this work, we analyze the performance of existing dialog models in situations where the input dialog context exhibits use of figurative language. We observe large gaps in handling of figurative language when evaluating the models on two open domain dialog datasets. When faced with dialog contexts consisting of figurative language, some models show very large drops in performance compared to contexts without figurative language. We encourage future research in dialog modeling to separately analyze and report results on figurative language in order to better test model capabilities relevant to real-world use. Finally, we propose lightweight solutions to help existing models become more robust to figurative language by simply using an external resource to translate figurative language to literal (non-figurative) forms while preserving the meaning to the best extent possible.

==> finaltodosList.tex <==


% H
% update figure > done
% remove comments from files > done
% remove redundant files and images > done
% see examples once more > done
% proof read. e.g. meteor vs METEOR  > done
% remove city names etc from references > done
% appendix review > done
    % removed mitigation examples table, since they are already there in the main paper
    % 
% final check on reviews > done


% V
% see examples once more
% proof read. e.g. meteor vs METEOR 
% final check on reviews
% delete todolist and reviews.text
% put on arxiv






==> reviews.tex <==




============================================================================ 
EMNLP 2021 Reviews for Submission #3465
============================================================================ 

Title: Investigating Robustness of Dialog Models to Popular Figurative Language Constructs
Authors: Harsh Jhamtani, Varun Gangal, Eduard Hovy and Taylor Berg-Kirkpatrick


============================================================================
                            REVIEWER #1
============================================================================

What is this paper about, what contributions does it make, and what are the main strengths and weaknesses?
---------------------------------------------------------------------------
This paper addresses the robustness of dialog models to the use of figurative language. To do so, the authors applied several existing general-purpose models to the DailyDialog and PersonaChat datasets and compared the performance achieved on the whole datasets with that achieved on the subsets consisting of the dialogs that contain figurative language. As expected, there was a drop in performance on those subsets, both in terms of automatic overlap metrics and human evaluation. Additionally, the authors have shown that the performance of the models can be recovered by replacing the segments containing figurative language by their literal counterparts. Finally, they proposed a lightweight automatic method to recover part of that performance, which uses a metaphor classifier and an idiomatic expression detector to identify segments containing figurative language and a lookup dictionary to provide the corresponding literal counterparts.

Overall, although the results were expected, I think it is an interesting short paper that raises awareness to the limitations of general-purpose language models. Furthermore, the authors provide the figurative language annotations and the literal equivalents, which simplify and promote future research in this area.
---------------------------------------------------------------------------


Reasons to accept
---------------------------------------------------------------------------
The paper raises awareness to the limitations of general-purpose language models when faced with figurative language and provides dialog annotations that promote future research in the area.
---------------------------------------------------------------------------


Reasons to reject
---------------------------------------------------------------------------
The results were expected and parts of the paper could be clearer.
---------------------------------------------------------------------------


Questions for the Author(s)
---------------------------------------------------------------------------
1 - The description of the datasets states that there are two literal versions of each sentence with figurative language. Are both of them used for evaluation?

2 - The mitigation approach leads to a much lower improvement on PersonaChat than on DailyDialog. What is the reason for this?
---------------------------------------------------------------------------


Typos, Grammar, Style, and Presentation Improvements
---------------------------------------------------------------------------
In the example in Figure 1, there are two segments of figurative language: "built on the sand" and "landed on the rocks". Although the focus is on the first, I think that the second one deserves at least a reference.

(Line 109): "most the prevalent" -> the most prevalent

(Table 1): There are % signs for the human evaluation, but not for the others.

In Tables 2 and 3, the approaches and results separated by / can be a bit confusing.

(Line 158): "Above analysis" -> The analysis above

(Lines 162-166): The description of the two scenarios is not totally clear.

(Line 199): "we skip using model" -> we skip using the model

(Line 205): "dilaog" -> dialog

(Line 248): "From Table 3" -> In Table 3

(Line 260): "there is scope of multiple future extensions" sounds weird

(Line 295): "similar direction" -> a similar direction

(Line 301): "analyzing capability" -> analyzing the capability
---------------------------------------------------------------------------


---------------------------------------------------------------------------
Reviewer's Scores
---------------------------------------------------------------------------
                         Reproducibility: 4
    Overall Recommendation - Short Paper: 3.5


============================================================================
                            REVIEWER #2
============================================================================

What is this paper about, what contributions does it make, and what are the main strengths and weaknesses?
---------------------------------------------------------------------------
This short paper shows that existing chatbot dialog models, such as
those based on fine-tuning GPT-2, continue to degrade performance in
the fact of figurative language including metaphors, idioms,
rhetorical questions, hyperbole, and "personalization" (Table 1).
Performance is correspondingly improved when such figures are replaced
by literal meanings (Table 2).  Datasets labeling figurative language
and providing literal alternatives, derived from DailyDialog and
PersonaChat, are offered.

The paper also presents a
semi-automatic mitigation mechanism for dealing with the first two
figurative categories.  The mitigation mechanism is based on automatic
detection of metaphors and idioms using existing classifiers, coupled
with Wiktionary look-up of literal meanings.  This mechanism is
necessarily limited to  
clichés and conventionalized or "frozen" varieties of metaphor, and is
rightly admitted not to handle novel metaphors or figures such as
sarcasm and hyperbole, but it has an ameliorating effect across the
board, particularly for DD-fig (the DD dialogs that include figurative
language).

The paper is interesting and well written.  The datasets will be useful
for evaluating semantic NLP programs, such as NLI and
text-entailment, as well as in building more robust chatbots.

Results seem solid, although the discussion is somewhat abbreviated,
perhaps from lack of space.  There is no explicit comparison of the
mitigation scheme in table 3 with the gold standard dataset in table
2.   In the case of DD-fig, recovery under some measures (including
human judgement) is a substantial proportion of the gold standard.  In
other cases (Blue 4) it is much less.  It is also odd that Rouge fails
to correlate with METEOR on the gold-standard table 2, but correlates
in table 3.

Minor points:

The motivating example in Figure 1 of GPT-2 misinterpreting "love built
on sand" is very clear and cute, but it is distracting that there is a second
metaphor/idiom in the opponent's input, namely "marriage landed on the rocks"
which is not shown as literalized.  Maybe comment or use another example
from Appendix F.

The references are somewhat non-standard, with abbreviations for
conference-names, missing page numbers, etc., and arXiv citations for
papers that have actually appeared in properly referreed conference
proceedings  (e.g. Devlin et al 2019 and Saleh et al, 2020).
---------------------------------------------------------------------------


Reasons to accept
---------------------------------------------------------------------------
see review
---------------------------------------------------------------------------


Reasons to reject
---------------------------------------------------------------------------
see review
---------------------------------------------------------------------------


Questions for the Author(s)
---------------------------------------------------------------------------
See review
---------------------------------------------------------------------------


Missing References
---------------------------------------------------------------------------
n/a
---------------------------------------------------------------------------


---------------------------------------------------------------------------
Reviewer's Scores
---------------------------------------------------------------------------
                         Reproducibility: 4
    Overall Recommendation - Short Paper: 3.5


============================================================================
                            REVIEWER #3
============================================================================

What is this paper about, what contributions does it make, and what are the main strengths and weaknesses?
---------------------------------------------------------------------------
In this paper the authors identify gaps in the handling of figurative language in dialog systems and propose approaches to address their handling. The authors begin with investigating the performance of popular models that have performed effectively on the DailyDialog dataset on a subset of the corpus containing conversations containing use of figurative language to measure how well figurative language is handled by those models. The authors further make use of the human annotated literal equivalents of the figurative contexts to measure the impact on performance. The authors further propose a lightweight mitigation model using literal translations from existing open source datasets. 
The strength of the paper is that it is comprehensive in experimentation and investigation of gaps and methods to handle figurative language in dialog systems which in my opinion is a relatively less researched area. If the authors make the datasets available to public it would encourage further research in the domain to improve its handling in dialog systems.
The weakness is that it uses existing state-of-the-art models in it's experiments although it does also introduce new ideas with literal forms.
---------------------------------------------------------------------------


Reasons to accept
---------------------------------------------------------------------------
Handling of figurative language in dialog systems is in my opinion a less researched area and this paper introduces initial research that can open up further avenues. The paper demonstrates several experiments and empirical results from different approaches. The dataset if released as open-source will be valuable to the community to continue further research in the area.
---------------------------------------------------------------------------


Questions for the Author(s)
---------------------------------------------------------------------------
1. After distilling the DailyDialog dataset for figurative language how many sentences comprise the DailyDialog-Figurative dataset?

2. In the mitigation approach in section 4, does the model suffer from a mismatch in domains and figurative between the VUA and DailyDialog datasets?
---------------------------------------------------------------------------


Missing References
---------------------------------------------------------------------------
Missing citations for VUA metaphor detection - 
1. Beata Beigman Klebanov, Chee Wee Leong, Michael Heilman, and Michael Flor. 2014. Different texts, same metaphors: Unigrams and beyond. In Proceedings of the Second Workshop on Metaphor in NLP, ACL.
2. Chee Wee Leong, Beata Beigman Klebanov, Chris Hamill, Egon Stemle, Rutuja Ubale, and Xianyang Chen. "A report on the 2020 vua and toefl metaphor detection shared task." In Proceedings of the Second Workshop on Figurative Language Processing, pp. 18-29. 2020.
---------------------------------------------------------------------------


Typos, Grammar, Style, and Presentation Improvements
---------------------------------------------------------------------------
"dialog" instead of dilaog on line 205
---------------------------------------------------------------------------


---------------------------------------------------------------------------
Reviewer's Scores
---------------------------------------------------------------------------
                         Reproducibility: 4
    Overall Recommendation - Short Paper: 3.5




